RECALL: A Benchmark for LLMs Robustness against External Counterfactual Knowledge

LLMs and AI chatbots have improved people's efficiency in various fields. However, the necessary knowledge for answering the question may be beyond the models' knowledge boundaries. To mitigate this issue, many researchers try to introduce external knowledge, such as knowledge graphs and Internet contents, into LLMs for up-to-date information. However, the external information from the Internet may include counterfactual information that will confuse the model and lead to an incorrect response. Thus there is a pressing need for LLMs to possess the ability to distinguish reliable information from external knowledge. Therefore, to evaluate the ability of LLMs to discern the reliability of external knowledge, we create a benchmark from existing knowledge bases. Our benchmark consists of two tasks, Question Answering and Text Generation, and for each task, we provide models with a context containing counterfactual information. Evaluation results show that existing LLMs are susceptible to interference from unreliable external knowledge with counterfactual information, and simple intervention methods make limited contributions to the alleviation of this issue.

==> tables/instructions.tex <==
\begin{table*}
    \centering
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cc|l}
    \toprule
         Dataset & \multicolumn{2}{c|}{Step} & Instruction \\
    \midrule
         \multirow{13}{*}{EventKG} & \multicolumn{2}{c|}{Paraphrase} & \makecell[l]{You are given the metadata about [EVENT] above. You should transform the metadata into natural language. Return the \\natural language text.} \\
         & \multicolumn{2}{c|}{QA} & \makecell[l]{You are given the metadata about [EVENT] above. You should generate a question that can be answered by one item in \\the metadata. Return the question and the key of the item containing the answer. Your output should be in JSON data format.} \\
         & \multicolumn{2}{c|}{Edit Answer} & \makecell[l]{You are given the metadata about [EVENT] above. You should change the value of item "[ATTRIBUTE]" to another different \\value that doesn't match the description in the metadata. Only return the edited item "[ATTRIBUTE]". Your output \\should be in JSON data format.} \\
         & \multirow{6}{*}{Edit Non-answers} & when & \makecell[l]{You are given a paragraph about [EVENT] above. You should change and only change the dates mentioned in the paragraph. \\Return the edited new paragraph. If the paragraph doesn't contain any time information, just return the original paragraph.} \\
         & & where & \makecell[l]{You are given a paragraph about {EVENT} above. Change one and only one name of city, country or continent appearing in the \\paragraph and return the edited new paragraph. If there are not any names of cities, countries or continents in the paragraph, \\just return the original paragraph.} \\
         & & who & \makecell[l]{You are given a paragraph about [EVENT] above. Change a person's name appearing in the paragraph to another different name \\and return the edited new paragraph. If there are not any people's names in the paragraph, just return the original paragraph.} \\
    \midrule
         \multirow{9}{*}{UJ} & \multicolumn{2}{c|}{Paraphrase} & \makecell[l]{You are given several sentences about [TERM] above. You should generate a summary that is as short as possible about [TERM] \\according to these sentences. You should remove all overlapping information from the summary.} \\
         & \multicolumn{2}{c|}{QA} & \makecell[l]{You are given a paragraph about [TERM] above. You should generate a question that can be answered by the paragraph. Return \\the question and corresponding answer. Your output should be in JSON data format. The question cannot be "What is [TERM]?" \\or any question with a similar meaning. The answer must be an original phrase that is as short as possible from the paragraph.} \\
         & \multicolumn{2}{c|}{Edit Answer} & \makecell[l]{You are given a question about [TERM] and the corresponding answer above. You should change some words in the answer \\to other words with totally different or opposite meanings. Only return the edited answer.} \\
         & Edit Non-answers & words & \makecell[l]{You are given several sentences about [TERM] above. For each sentence, you should change one and only one word/phrase in it \\to another word/phrase with a totally different or opposite meaning. Return the edited sentences. Your output should be in JSON \\data format.} \\         
    \bottomrule
    \end{tabular}
    }
    \caption{The instructions we use during constructing the benchmark.}
    \label{tab:instruction}
\end{table*}


